CARL: A Benchmark for Contextual and Adaptive Reinforcement Learning

While Reinforcement Learning has made great strides towards solving ever more complicated tasks, many algorithms are still brittle to even slight changes in their environment. This is a limiting factor for real-world applications of RL. Although the research community continuously aims at improving both robustness and generalization of RL algorithms, unfortunately it still lacks an open-source set of well-defined benchmark problems based on a consistent theoretical framework, which allows comparing different approaches in a fair, reliable and reproducibleway. To fill this gap, we propose CARL, a collection of well-known RL environments extended to contextual RL problems to study generalization. We show the urgent need of such benchmarks by demonstrating that even simple toy environments become challenging for commonly used approaches if different contextual instances of this task have to be considered. Furthermore, CARL allows us to provide first evidence that disentangling representation learning of the states from the policy learning with the context facilitates better generalization. By providing variations of diverse benchmarks from classic control, physical simulations, games and a real-world application of RNA design, CARL will allow the community to derive many more such insights on a solid empirical foundation.

==> acknowledgements.tex <==
\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2021/PaperInformation/FundingDisclosure}.

Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{sec:limitations}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{No theoretical results.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{No theoretical results so no proofs.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Section~\ref{sec:experiments}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section~\ref{appendix:hardhyper} in the appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{Apache 2.0 as stated in the github repository.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{No dataset collected.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{No crowdsourcing or research with human subjects.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> latexmkrc <==

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

$bibtex='bibtex -min-crossrefs=20'

==> tables/context_features/context_features_defaults_bounds_CARLHalfcheetah.tex <==
\begin{subtable}{0.4\textwidth}
\centering
\caption[CARLHalfcheetah]{CARLHalfcheetah}
\label{tab:context_features_defaults_bounds_CARLHalfcheetah}
\begin{tabular}{lrll}
\toprule
      Context Feature &  Default &       Bounds &  Type \\
\midrule
      angular\_damping &    -0.05 &  (-inf, inf) & float \\
             friction &     0.60 &  (-inf, inf) & float \\
              gravity &    -9.80 & (-inf, -0.1) & float \\
joint\_angular\_damping &    20.00 &     (0, inf) & float \\
      joint\_stiffness & 15000.00 &     (1, inf) & float \\
           torso\_mass &     9.46 &   (0.1, inf) & float \\
\bottomrule
\end{tabular}
\end{subtable}


==> tables/context_features/context_features_defaults_bounds_CARLMountainCarContinuousEnv.tex <==
\begin{subtable}{0.4\textwidth}
\centering
\caption[CARLMountainCarContinuousEnv]{CARLMountainCarContinuousEnv}
\label{tab:context_features_defaults_bounds_CARLMountainCarContinuousEnv}
\begin{tabular}{lrll}
\toprule
   Context Feature &  Default &      Bounds &  Type \\
\midrule
     goal\_position &     0.45 & (-inf, inf) & float \\
     goal\_velocity &     0.00 & (-inf, inf) & float \\
      max\_position &     0.60 & (-inf, inf) & float \\
max\_position\_start &    -0.40 & (-inf, inf) & float \\
         max\_speed &     0.07 &    (0, inf) & float \\
max\_velocity\_start &     0.00 & (-inf, inf) & float \\
      min\_position &    -1.20 & (-inf, inf) & float \\
min\_position\_start &    -0.60 & (-inf, inf) & float \\
min\_velocity\_start &     0.00 & (-inf, inf) & float \\
             power &     0.00 & (-inf, inf) & float \\
\bottomrule
\end{tabular}
\end{subtable}


==> tables/context_features/context_features_defaults_bounds_CARLUr5e.tex <==
\begin{subtable}{0.4\textwidth}
\centering
\caption[CARLUr5e]{CARLUr5e}
\label{tab:context_features_defaults_bounds_CARLUr5e}
\begin{tabular}{lrll}
\toprule
      Context Feature &  Default &       Bounds &  Type \\
\midrule
    actuator\_strength &   100.00 &     (1, inf) & float \\
      angular\_damping &    -0.05 &  (-inf, inf) & float \\
             friction &     0.60 &  (-inf, inf) & float \\
              gravity &    -9.81 & (-inf, -0.1) & float \\
joint\_angular\_damping &    50.00 &     (0, 360) & float \\
      joint\_stiffness & 40000.00 &     (1, inf) & float \\
      target\_distance &     0.50 &  (0.01, inf) & float \\
        target\_radius &     0.02 &  (0.01, inf) & float \\
           torso\_mass &     1.00 &     (0, inf) & float \\
\bottomrule
\end{tabular}
\end{subtable}


==> tables/overview_benchmarks.tex <==
\newcolumntype{P}[1]{>{\raggedright\arraybackslash}p{#1}}
\begin{table}[]
    \small{
    \centering
    \caption{Benchmark collections in Meta-RL}
    \label{tab:overview_benchmarks_related_work}
    \begin{tabular}{P{2cm}P{2.3cm}P{2.5cm}P{2.3cm}P{2cm}}
    \toprule
        Benchmark &  Goal & Environments & Variations of the Task & Access \\
        \midrule
        \addlinespacetable
        MDP Playground~\citep{rajan-arxiv19} 
        & AutoRL \& Characterization of RL algorithms 
        & Toy settings \& MuJoCo/Atari extensions
        & Properties of RL problems (e.g. reward delay) 
        & open-source (except for MuJoCo wrapper)  \\
        %\hline
        bsuite ~\citep{osband-iclr20} 
        & Characterization of RL algorithms 
        & Bandits \& Classic Control
        & Fixed experiments
        & open-source
        \\
        %\hline
        \addlinespacetable
        ALE \citep{machado-jair28} 
        & Transfer within ALE tasks
        & Arcade game environments
        & Fixed experiments (flavors)
        & open-source \\
        %\hline
        \addlinespacetable
        ProcGen \citep{cobbe-2019} 
        & Generalization
        & Arcade Games 
        & Procedurally generated levels
        & open-source \\
        %\hline
        \addlinespacetable
        Alchemy \citep{wang-corr21} 
        & Generalization \& skill acquisition
        & Standard and simplified alchemy environment
        & Distribution across levels
        & open-source\\
        %\hline
        \addlinespacetable
        Meta-world \citep{yu-corl19} 
        & Transfer Learning 
        & Hand Manipulation tasks
        & Standardized sets of tasks
        & closed-source (MuJoCo required)\\
        %\hline
        \addlinespacetable
        MTEnv \citep{sodhani-2021} 
        & Transfer Learning, Representation Learning \& Generalization
        & Toy Settings, Meta-world, Block MDP enironments
        & Fixed settings
        & closed-source (MuJoCo required)\\
        %\hline
        \addlinespacetable
        Safety Gym \citep{ray-2019} 
        & Safe RL
        & Robot navigation with hazards
        & Several configurable features per task
        & closed-source (MuJoCo required)\\
        %\hline
        \addlinespacetable
        TeachMyAgent \citep{romac-icml21} 
        & Student-Teacher Curriculum Learning
        & Box2D tasks with several different walkers each
        & Task distribution with increasing difficulty
        & open-source\\
        %\hline
        \addlinespacetable
        Offworld Gym \citep{offworldgym} 
        & Training on a real robot
        & Robot navigation
        & Discrete \& continuous
        & open-source \\
        %\hline
        \midrule
        \addlinespacetable
        \GenRL (ours)
        & Generalization
        & Classic Control, Box2D, Brax robots, game playing, RNA design
        & Several configurable features per task
        & open-source \\
    \bottomrule
    \end{tabular}
    }
\end{table}
